Verifying C11-Style Weak Memory Libraries

Deductive verification of concurrent programs under weak memory has thus far been limited to simple programs over a monolithic state space. For scalabiility, we also require modular techniques with verifiable library abstractions. This paper addresses this challenge in the context of RC11 RAR, a subset of the C11 memory model that admits relaxed and release-acquire accesses, but disallows, so called, load-buffering cycles. We develop a simple framework for specifying abstract objects that precisely characterises the observability guarantees of abstract method calls. We show how this framework can be integrated with an operational semantics that enables verification of client programs that execute abstract method calls from a library it uses. Finally, we show how implementations of such abstractions in RC11 RAR can be verified by developing a (contextual) refinement framework for abstract objects. Our framework, including the operational semantics, verification technique for client-library programs, and simulation between abstract libraries and their implementations, has been mechanised in Isabelle/HOL.

==> composition.tex <==
\section{Client library composition}

While the verification Key to our paper is the observation that one can compose clients and
objects


==> view-relaxation.tex <==
\newcommand{\ww}{{\it ww}}
\newcommand{\tts}{{\it tt}}
\section{Exploiting View-based relaxation}
\label{sec:view-based-relax}

The modelling approach in \refsec{sec:abstr-object-semant} provides a
flexible framework for specifying abstract objects and enables
specification of synchronised and unsynchronised method calls (as
detailed in Figs.~\ref{fig:publication} and \ref{fig:rfs}). We show that the framework also provides a
mechanism for specifying concurrent objects whose linearisation order
is different from real-time order (cf 
\cite{DBLP:journals/pacmpl/RaadDRLV19,DongolJRA18,DBLP:conf/esop/KrishnaEEJ20,DBLP:journals/pacmpl/EmmiE19}).
% In this section, we present some design choices for concurrent stacks
% and queues. 
% In particular, we show that it is possible (using
% thread-local views) to describe the behaviour of abstract objects
% where operations take effect in an order different from real-time
% order. 
We argue that such specifications are a natural fit with the
weak memory operational semantics where new writes may be introduced
in the ``middle'' of modification
order~\cite{DBLP:conf/ppopp/DohertyDWD19,Dolan:2018:LDRF,DBLP:conf/popl/KangHLVD17}. Of
course, such relaxations do not apply to every shared object, e.g.,
locks (\refex{ex:abs-lock}).

 % This is
% analogous to the idea that different threads may have different views
% of writes to each variable in C11 memory
% models~\cite{DBLP:conf/ecoop/KaiserDDLV17,ECOOP20,DBLP:conf/popl/KangHLVD17}. From
% the perspective of client-library synchronisation, we aim to provide
% per-method visibility-based notions of consistency defined in prior
% work~\cite{DongolJRA18,DBLP:journals/pacmpl/EmmiE19}. % However, we also
% % aim to allow optimisations already present 


% For data structures like a queue stack, modification methods such as a
% push are inherently \GVar_C \lhd

% We require that the linear order is consistent with the object's
% sequential specification (as required by linearizability
% \cite{DongolJRA18,HeWi90}), but only guarantee consistency up to the
% minimal viewfront for all threads. That is, we consider the views of
% all threads of the shared object and only require consistency of
% method calls (with respect to the sequential specification) up to the
% the minimal view, i.e., for a prefix of the method calls recorded for
% the object. This means that once all views ``catch up'' to the last
% method call (in timestamp order), the full sequence of calls is
% guaranteed to be consistent with a sequential specification. 

As with writes, timestamps may be used to define a linear order of the
method calls of the object in question. However, \emph{different}
threads may have to have \emph{different} views of the object being
implemented, even at the level of the abstraction. % Consider a few
% key data structures.

For example, consider the state of a shared queue depicted below
\begin{center}
  \begin{tikzpicture}[scale=0.65]
    \draw[thick,->] (-1,0) -- (7,0);
        
    \coordinate (init) at (-1,0);
    \coordinate (enq1) at (1,0);
    \coordinate (enq2) at (3.5,0);
    \coordinate (deq2) at (6,0);
    
    % \coordinate (T1-1) at (5,4); \coordinate (T2-1) at (5,2.5);
    
    % \draw (0,4) node[above] {$d$}; \draw (1.5,4) node[above] {$f$};
    % \draw (T1-1) node[above] {T1 view}; \draw (T2-1) node[above] {T2
    % view};
    
    \draw (init) circle (4pt)
    node[below]  {$\initq()$};

    % \draw (enq1) circle (4pt)
    % node[below]  {$enq(1)$}
    % node[above]  {$t_1$};

    \draw (enq1) circle (4pt)
    node[below]  {$\enq(1)$}
    node[above]  {$t_1$};
    
    \draw [black] (enq2) circle (4pt)
    node[below]  {$\enq(2)$};
    
    \draw [black] (deq2) circle (4pt)
    node[below]  {$\deq(v)$} 
    node[above]  {$t_2$};

    % \filldraw [black] (pop1) circle (2pt)
    % node[below]  {$pop(x)$};
    
  \end{tikzpicture}
\end{center}
where the viewfront of threads $t_1$ and $t_2$
are depicted above the timeline and the abstract operations executed
below the timeline. The execution may have been generated by executing
the operations in the following temporal order:
\begin{enumerate}
\item Thread $t_2$ executes $\enq(2)$, and hence $t_2$'s view of the
  data structure should be that of $\enq(2)$.
\item Thread $t_1$ executes $\enq(1)$, but since it has not yet
  ``seen'' $\enq(2)$, it may choose a timestamp that is smaller than
  the timestamp of $\enq(2)$ for $enq(1)$.
\item Thread $t_2$ executes a dequeue, $\deq(v)$, for some yet to be
  determined value $v$. Since $t_2$ also executed $\enq(2)$, the
  timestamp of the $\deq(v)$ must be larger than that of
  $\enq(2)$. Since the timeline represents a linearization of the
  queue, the only sensible value for $v$ is $1$.
\end{enumerate}
One option for the execution to continue in a sensible manner is to
ensure that the effect of the dequeue is communicated to all other
threads so that their views of the object are updated. Thus, if $t_1$
were to perform a new method call, this method call would appear after
$\deq(v)$ (with $v = 1$). However, imposing such a communication
requirement in the abstract specification induces additional (and
potentially unnecessary) synchronisation in an implementation. For
instance, a sensible continuation of the timeline in above would be
for thread $t_1$ to introduce additional enqueue operations between
$\enq(1)$ and $\deq(v)$ (with $v = 1$). % In fact, the only
% continuations that are disallowed is the introduction of new dequeue
% operations between $\enq(1)$ and $\deq(v)$ and new enqueue operations
% before $\enq(1)$.



% The question now is: what are the acceptable values for $v$? One
% option is to require this dequeue to return $1$ to globally maintain
% queue consistency. However, imposing such a requirement means that
% thread $t_1$ is no longer be able to insert a dequeue between $enq(1)$
% and $enq(2)$. The only way to guarantee this is to communicate the
% effect of the dequeue by thread $t_2$ to $t_1$ so that $t_1$'s view of
% the queue can be updated. On one hand, this seems a sensible
% requirement, however, it also means that it also induces additional
% synchronisation on the implementation of the data structure.

% \begin{figure}[t]
%   \centering
  
%   \begin{minipage}[t]{0.45\columnwidth}
%   \caption{Possible timeline of queue data structure}
%   \label{fig:lin-order}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.45\columnwidth}
%   \begin{tikzpicture}[scale=0.65]
%     \draw[thick,->] (-1,0) -- (7,0);
        
%     \coordinate (init) at (-1,0);
%     \coordinate (enq1) at (1,0);
%     \coordinate (enq2) at (3.5,0);
%     \coordinate (deq2) at (6,0);
    
%     % \coordinate (T1-1) at (5,4); \coordinate (T2-1) at (5,2.5);
    
%     % \draw (0,4) node[above] {$d$}; \draw (1.5,4) node[above] {$f$};
%     % \draw (T1-1) node[above] {T1 view}; \draw (T2-1) node[above] {T2
%     % view};
    
%     \draw (init) circle (4pt)
%     node[below]  {$\initq()$};

%     % \draw (enq1) circle (4pt)
%     % node[below]  {$enq(1)$}
%     % node[above]  {$t_1$};

%     \filldraw (enq1) circle (4pt)
%     node[below]  {$\enq(1)$}
%     node[above]  {$t_1$};
    
%     \draw [black] (enq2) circle (4pt)
%     node[below]  {$\enq(2)$};
    
%     \draw [black] (deq2) circle (4pt)
%     node[below]  {$\deq(v)$} 
%     node[above]  {$t_2$};

%     % \filldraw [black] (pop1) circle (2pt)
%     % node[below]  {$pop(x)$};
    
%   \end{tikzpicture}
%   \caption{Queue timeline with covered operations}
%   \label{fig:lin-order-covered}
% \end{minipage}
  
% \end{figure}



% We address this issue by extending the notion of a covered operation
% as used for read-modify write updates (see \reffig{fig:surrey-opsem})
% and use it to establish atomicity between the operation that is
% covered and another corresponding operation. The precise details of
% the interaction between covering and the method calls of the data
% structure will be specific to the data structure at hand.

\begin{example}[Queue data structure]
  For simplicity, we assume a new state component, $\matchedTS$, that
  stores the pairs of timestamps corresponding to enqueues that have
  been dequeued. For any $(ts, ts') \in \matchedTS$, the timestamp
  $ts$ corresponds to an enqueue that is removed from the queue by the
  dequeue with timestamp $ts'$. To ensure first-in-first-out
  behaviours, for any pair $(ts, ts') \in \matchedTS$, it is illegal
  for a dequeue to be introduced between $ts$ and $ts'$. Note that
  $\matchedTS$ can be calculated from any queue state so its
  introduction only plays an auxiliary role.

  Below, we present a specification of \emph{synchronising} enqueue
  and dequeue operations. It is straightforward to extend these to
  also specify unsynchronised accesses (see \reffig{fig:rfs}).
  % In a queue data structure, the effect of a dequeue method is to
  % \emph{cover} the associated enqueue that the dequeue interacts with and its
  % meaning is to disallow intervening dequeues that return a queued
  % value between the enqueue and this dequeue. % Moreover, we require
  % % that the initialisation is covered and that a dequeue that returns
  % % empty may be introduced after a covered write. 
  % Finally, an enqueue
  % must not be introduced before another covered enqueue
  % operation. Using filled circles to denote covered operations, the
  % introduction of covering to the timeline in \reffig{fig:lin-order}
  % results in the timeline given in \reffig{fig:lin-order-covered}, and
  % the expected behaviour is ensured by the following rules.
\[ \inference[{\sc Enq}] {
    a \in q.enq_u % \qquad (w, \ts) \in \gamma.\OW(t, x) % \setminus \gamma.\covered
    \qquad 
    \tst(\gamma.\tview_t(q)) < \ts' \qquad     \writes' = \gamma.\writes \cup \{(a, \ts')\} \\
    (\forall (\mathit{ww}, \mathit{tt}) \in \gamma.\writes.\
    \ww \in Enq \wedge \tts > \ts'  \imp \mathit{tt} \notin \dom(\gamma.\matchedTS))
    % \{   \mid \ts' < \mathit{tt} \wedge \mathit{ww} \in Enq\} \cap \gamma.\covered = \emptyset
    \\
    (\forall (\ww, \tts) \in \gamma.\writes.\ \tts > \ts' \imp ww \noteq q.deq_{\it empty}) \\
    \mview' = \tview' \cup \beta.\tview_t \qquad 
    \tview' = \gamma.\tview_t[q := (a, \ts')]  
  }
  {\gamma, \beta\  \strans{a}_{t}\  \gamma[\writes \asgn \writes', \tview_t \asgn \tview', \mview_{(a,\ts')} \asgn \mview'], \beta }\\
\]\smallskip
\[  \inference[{\sc Deq-NE}] {
    a \in q.deq_u \qquad u \neq {\it empty} \qquad \tst(\gamma.\tview_t(q)) < \ts' \qquad \writes' = \gamma.\writes \cup \{(a, \ts')\}\\
    (w, \ts) \in \gamma.\writes \qquad \ts \notin \dom(\gamma.\matchedTS)  
    \\ 
    (\forall (\ww, \tts) \in \gamma.\writes.\ \tts \in Enq \wedge \tts < \ts \imp \tts \in \sigma.\matchedTS) \\
    (\forall \tts' \in \ran(\gamma.\matchedTS).\ ts' \geq \tts')
    \qquad
    \tview' = \gamma.\tview_t[q := (a, \ts')]  \otimes \gamma.\mview_{(w,\ts)}
    \\
    \ctview' = \beta.\tview_t  \otimes \gamma.\mview_{(w,\ts)}
  }
  {\gamma, \beta\  \strans{a}_{t}\  \gamma[\writes \asgn \writes', \tview_t \asgn \tview', \mview_{(a,\ts')} \asgn \mview'], \beta[\tview_t := \ctview']}\\
\]\smallskip
\[ \inference[{\sc Deq-Emp}] {
    a \in q.deq_{\it empty} \qquad \tst(\gamma.\tview_t(q)) < \ts' \qquad \writes' = \gamma.\writes \cup \{(a, \ts')\}\\
    (\forall (\ww, \tts) \in \gamma.\writes.\ \tts < \ts'
      \imp  \tts \in \dom(\sigma.\matchedTS) \cup \ran(\sigma.\matchedTS) \lor \ww = q.deq_{\empty})
\\
    \tview' = \gamma.\tview_t[q := (a, \ts')] %   \otimes \gamma.\mview_{(w,q)}
  }
  {\gamma, \beta\  \strans{a}_{t}\  \gamma[\writes \asgn \writes',
    \tview_t \asgn \tview'], \beta }
\]

\smallskip Thus, enqueues and dequeues must not interfere with other dequeue
operations that have already taken effect, including dequeue
operations that return empty. The behaviour of enqueue operations is
analogous to releasing writes, whereas the behaviour of non-empty
dequeue operations is analogous to read-modify-write operations.
\end{example}

Given that a dequeue that returns empty only observes the queue and
does not modify it, one could argue that such operations are analogous
to reads, and hence, should not appear in the timeline at all. Using
such a specification may allow non-atomic observations, leading to
phenomena observed by Emmi and Enea
\cite{DBLP:journals/pacmpl/EmmiE19}. We consider further exploration
of such ideas to be  future work.


% We argue that such a specification allows a simple to understand correctness notion 


 
% \bd{Yet, we support expected paradigms, e.g., message passing of
%   clients as well as\\ This makes our condition different from
%   \cite{DBLP:journals/pacmpl/RaadDRLV19}, who allow non-deterministic
%   abstract specifications to enable characterisation of specific
%   implementations, e.g., as found in the elimination
%   stack~\cite{DBLP:journals/jpdc/HendlerSY10}.}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

